MEEK: Re-thinking Heterogeneous Parallel Error Detection Architecture for Real-World OoO Superscalar Processors

Heterogeneous parallel error detection is an approach to achieving fault-tolerant processors, leveraging multiple power-efficient cores to re-execute software originally run on a high-performance core. Yet, its complex components, gathering data cross-chip from many parts of the core, raise questions of how to build it into commodity cores without heavy design invasion and extensive re-engineering. We build the first full-RTL design, MEEK, into an open-source SoC, from microarchitecture and ISA to the OS and programming model. We identify and solve bottlenecks and bugs overlooked in previous work, and demonstrate that MEEK offers microsecond-level detection capacity with affordable overheads. By trading off architectural functionalities across codesigned hardware-software layers, MEEK features only light changes to a mature out-of-order superscalar core, simple coordinating software layers, and a few lines of operating-system code. The Repo. of MEEK's source code: https://github.com/SEU-ACAL/reproduce-MEEK-DAC-25.

==> Outline.tex <==



\zhenote{Please remember to introduce the progress of parallel and heterogeneous error detection in an early place, including the concepts of ``checkpoints'', etc.}

\noindent \textbf{Backgrounds:} 
\begin{itemize}
    \item (1) Lockstep is widely used in the [automotive industry, but should also be general].
    While it is safe, it is also very expensive -- consuming more than 2x hardware; 
    
    \item (2) Heterogeneous and parallel error detection has been seen as a competitive candidate for the lockstep. 
    However, since Diva was proposed in year 1999, until ParaMedic was developed in year 2019, there is still none of the heterogenous and parallel error detection. 
\end{itemize}

\noindent \textbf{Challanges:}  Heterogeneous and parallel error detection remains an emerging concept, however the method to build it in real is still unknown, because there is a missing of
\begin{itemize}
    \item (I) microarchitecture at hardware level;
    \item (II) programming model at software level;
    \item (III) a systematic framework as a complete solution.
\end{itemize}

\textbf{Contributions:} 
In this paper, we propose \name{}, ....
\zhenote{What are the benefits of each of them?}
\begin{itemize}
    \item (I) microarchitecture
    \item (II) New ISA: custom\_jalr, etc.
    \item (III) Programming model 
    \item (IV) A full-stack solution, from microarchitecture and architecture to ISA and programming model.
\end{itemize}


\zhenote{To do: write this paepr, first.\\}
\zhenote{To do: read DSN'19, and list the problems.}



\begin{table*}[]
\begin{tabular}{l|l|l}
\hline
                                                                     & \textbf{DSN'18}                                                                                                         & \textbf{PyraMedic}                                                                                                  \\ \hline
Scheme Overview                                                      & \cellcolor[HTML]{FFCCC9}Pure Hardware Scheme                                                                            & \cellcolor[HTML]{9AFF99}Hardware/Software Co-design                                                                 \\ \hline
Checker Core                                                         & \cellcolor[HTML]{FFCCC9}Check-only                                                                                      & \cellcolor[HTML]{9AFF99}Checker/application core                                                                    \\ \hline
Flexibility                                                          & \cellcolor[HTML]{FFCCC9}Fixed                                                                                           & \cellcolor[HTML]{9AFF99}\begin{tabular}[c]{@{}l@{}}Configurable due to introductions\\ of new ISAs -- support lots of software schemes can be run \\ on the checker core, e.g., rollback, etc. \end{tabular}     \\ \hline
OS Supported                                                         & \cellcolor[HTML]{FFCCC9}No                                                                                              & \cellcolor[HTML]{9AFF99}Yes                                                                                         \\ \hline
Cover of ld data                                                     & \cellcolor[HTML]{9AFF99}\textbf{\begin{tabular}[c]{@{}l@{}}Yes, by forwarding data \\ directly from L1\$D\end{tabular}} & \cellcolor[HTML]{FFCCC9}\textbf{\begin{tabular}[c]{@{}l@{}}No,by forwarding data from \\ commit stage (ECC is covered) \end{tabular}} \\ \hline
Speculation handling                                                 & \cellcolor[HTML]{FFCCC9}\begin{tabular}[c]{@{}l@{}}Yes, handled by load-forwarding\\ Unit\end{tabular}                  & \cellcolor[HTML]{9AFF99}\begin{tabular}[c]{@{}l@{}}No, because we handle it at \\ commit stage\end{tabular}         \\ \hline
\begin{tabular}[c]{@{}l@{}}Cover non-repeatable\\ insts\end{tabular} & \cellcolor[HTML]{FFCCC9}No                                                                                              & \cellcolor[HTML]{9AFF99}Yes                                                                                         \\ \hline
Cover Atomic insts                                                   & \cellcolor[HTML]{FFCCC9}Unknown                                                                                         & \cellcolor[HTML]{9AFF99}Yes                                                                                         \\ \hline
\end{tabular}
\end{table*}


\textcolor{red}{DSN'18 is overly complicated due to overlook the micro-architecture -- maybe, our design does not involve any design invasion of the OoO superscalar core?.}

\clearpage



==> Preliminaries.tex <==
\begin{figure*}[t]   
    \centering
    \includegraphics[width=1\textwidth]{graphics/Overview.pdf}
    \vspace{-15pt}
    \caption{An overview of \name. \emph{(DEU: Data Extraction Unit; LSQ: Load-Store Queue; PRFs: Physical Register Files; CSRs: Control and Status Registers; HM-NoC: Half-duplex Multicast Network-on-Chip; MSU: Mode Switch Unit; L\$: Log Cache; M-Bus: Memory Bus)}. At hardware: \circled{a} a non-intrusive DEU is deployed in the big core, collecting data from various locations without disrupting the core's execution;
    \circled{b} a superscalar F$^2$ is developed, prioritizing and distributing the data only to the relevant little cores;
    \circled{c} dual-mode little cores are designed for correctness checking or workload execution.
    At software: \circled{d} a customized ISA abstracts the control interface for \circled{e}, the scheduler in the OS, enabling flexible management of verification and workload execution on the little cores.
    \vspace{-15pt}
    }
    \label{fig:AnOverview}
\end{figure*}



\section{Heterogeneous Parallel Error Detetion}
\label{sc:Preliminaries}
% Before diving into the technical details of \name, we first review the basic architecture with the challenges for real-world deployments.
\zhenote{Restricted to the 6-page limits, suggesting to remove this section. Instead, we can move some of the content in the intro.}


\subsection{Basic Architecture}
\label{sbsc:HP-ErrorDetection}
The key insight of heterogeneous parallel error detection is rooted in the fact that running code a second time is more readily parallelized than the original execution.
By taking periodic RCPs, the execution of a program on a high-performance big core is segmented into discrete portions that can be concurrently and independently verified.
This allows multiple power-efficient little cores to re-execute and verify different segments in an overlapping manner, collectively providing enough computational capacity to keep pace with the big core.

To allow a precise replay of memory and non-repeatable operations, the addresses and data of \texttt{load}, \texttt{store}, and other non-repeatable instructions are sequentially extracted from the program stream at the commit stage within the big core, generating a load-store log.
This log is partitioned and evenly distributed across the little cores.
When the load-store log of a segment is fulfilled, or an instruction timeout is reached, a new RCP is triggered, and the corresponding little core begins verifying the segment between the previous and current CRPs, designated as the Start RCPs (SRCPs) and End RCPs (ERCPs) of the little cores.
This asynchronous and distributed verification realizes the error detection with significantly less overheads compared to the conventional locksteps.

% ensures error detection is achieved with significantly less overheads compared to the conventional locksteps.



% Heterogeneous parallel error detection is a fault-tolerant architecture for the processor cores, offering a competitive alternative to the conventional dual-core lockstep~\cite{de2018lockstep,iturbe2016triple}. The architecture leverages strong induction and parallelism to divide the software program running on the OoO superscalar core (big core) into multiple segments and re-execute them concurrently on the smaller, low-power cores (little cores) to verify the execution correctness. By replicating Register Check Points (RCPs) and re-executing all instructions during the original execution of the program segments, spitted by the Start RCPs (SRCPs) and End RCPs (ERCPs), error detection can be achieved with significantly less overhead over the dual-core lockstep.




\subsection{Challenges for Making the Architecture in Real}
\label{sbsc:Challanges}
As described above, replaying program segments on different cores requires duplicating architectural states at each RCP and logging all memory and non-repeatable operations during execution.
This means that a huge volume of relevant data must be continuously collected from the big core, handling the parallel instruction commitments, all within a very narrow time window before subsequent instructions overwrite the data.
This also means that the collected data must be prioritized and routed to the corresponding little cores in real-time, to prevent the backpressure from stalling the big core's execution.
Even with the necessary data, the system must provide flexibility for the little cores' scheduling and management, as the applications often need different numbers of little cores for verification. 
Coarse-grained management could lead to inefficient verification or resource waste.

However, the architecture's hardware-only nature brings significant microarchitectural complexity and restricted system flexibility.
Since the architecture was conceptually presented in DIVA~\cite{austin1999diva} and in-depth investigated in a series of ParaMedic-style work~\cite{ainsworth2018parallel,ainsworth2019paramedic}, all prototypes have been studied using highly abstracted simulations, only validating its theoretical potential, leaving a gap to make it in real.
Here, we take all these challenges forward to develop \name\, the first systematical solution for heterogeneous parallel error detection.


==> refs.tex <==
% Encoding: UTF-8
@inproceedings{didehban2016nzdc,
  title={nZDC: A compiler technique for near zero silent data corruption},
  author={Didehban, Moslem and Shrivastava, Aviral},
  booktitle={Proceedings of the 53rd Annual Design Automation Conference},
  pages={1--6},
  year={2016}
}

@article{powell2009architectural,
  title={Architectural core salvaging in a multi-core processor for hard-error tolerance},
  author={Powell, Michael D and Biswas, Arijit and Gupta, Shantanu and Mukherjee, Shubhendu S},
  journal={ACM SIGARCH Computer Architecture News},
  volume={37},
  number={3},
  pages={93--104},
  year={2009},
  publisher={ACM New York, NY, USA}
}



@inproceedings{romanescu2008core,
  title={Core cannibalization architecture: improving lifetime chip performance for multicore processors in the presence of hard faults},
  author={Romanescu, Bogdan F and Sorin, Daniel J},
  booktitle={Proceedings of the 17th international conference on Parallel architectures and compilation techniques},
  pages={43--51},
  year={2008}
}

@article{yang2024efficient,
  title={An efficient multi-task learning CNN for driver attention monitoring},
  author={Yang, Dawei and Wang, Yan and Wei, Ran and Guan, Jiapeng and Huang, Xiaohua and Cai, Wei and Jiang, Zhe},
  journal={Journal of Systems Architecture},
  volume={148},
  pages={103085},
  year={2024},
  publisher={Elsevier}
}

@article{veeraraghavan2012doubleplay,
  title={DoublePlay: Parallelizing sequential logging and replay},
  author={Veeraraghavan, Kaushik and Lee, Dongyoon and Wester, Benjamin and Ouyang, Jessica and Chen, Peter M and Flinn, Jason and Narayanasamy, Satish},
  journal={ACM Transactions on Computer Systems (TOCS)},
  volume={30},
  number={1},
  pages={1--24},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gupta2008stagenet,
  title={The stagenet fabric for constructing resilient multicore systems},
  author={Gupta, Shantanu and Feng, Shuguang and Ansari, Amin and Blome, Jason and Mahlke, Scott},
  booktitle={2008 41st IEEE/ACM International Symposium on Microarchitecture},
  pages={141--151},
  year={2008},
  organization={IEEE}
}

@inproceedings{li2009mcpat,
  title={McPAT: An integrated power, area, and timing modeling framework for multicore and manycore architectures},
  author={Li, Sheng and Ahn, Jung Ho and Strong, Richard D and Brockman, Jay B and Tullsen, Dean M and Jouppi, Norman P},
  booktitle={Proceedings of the 42nd annual ieee/acm international symposium on microarchitecture},
  pages={469--480},
  year={2009}
}

@book{love2010linux,
  title={Linux kernel development},
  author={Love, Robert},
  year={2010},
  publisher={Pearson Education}
}

@article{aas2005understanding,
  title={Understanding the Linux 2.6. 8.1 CPU scheduler},
  author={Aas, Josh},
  journal={Retrieved Oct},
  volume={16},
  pages={1--38},
  year={2005}
}

@book{bovet2005understanding,
  title={Understanding the Linux Kernel: from I/O ports to process management},
  author={Bovet, Daniel P and Cesati, Marco},
  year={2005},
  publisher={" O'Reilly Media, Inc."}
}

@inproceedings{hameed2010understanding,
  title={Understanding sources of inefficiency in general-purpose chips},
  author={Hameed, Rehan and Qadeer, Wajahat and Wachs, Megan and Azizi, Omid and Solomatnikov, Alex and Lee, Benjamin C and Richardson, Stephen and Kozyrakis, Christos and Horowitz, Mark},
  booktitle={Proceedings of the 37th annual international symposium on Computer architecture},
  pages={37--47},
  year={2010}
}

@article{stolt2008design,
  title={Design and implementation of the POWER6 microprocessor},
  author={Stolt, Benjamin and Mittlefehldt, Yonatan and Dubey, Sanjay and Mittal, Gaurav and Lee, Mike and Friedrich, Joshua and Fluhr, Eric},
  journal={IEEE Journal of Solid-State Circuits},
  volume={43},
  number={1},
  pages={21--28},
  year={2008},
  publisher={IEEE}
}

@article{gao2015survey,
  title={A survey of fault diagnosis and fault-tolerant techniques—Part I: Fault diagnosis with model-based and signal-based approaches},
  author={Gao, Zhiwei and Cecati, Carlo and Ding, Steven X},
  journal={IEEE transactions on industrial electronics},
  volume={62},
  number={6},
  pages={3757--3767},
  year={2015},
  publisher={IEEE}
}

@article{schroeder2009dram,
  title={DRAM errors in the wild: a large-scale field study},
  author={Schroeder, Bianca and Pinheiro, Eduardo and Weber, Wolf-Dietrich},
  journal={ACM SIGMETRICS Performance Evaluation Review},
  volume={37},
  number={1},
  pages={193--204},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{hernandez2015timely,
  title={Timely error detection for effective recovery in light-lockstep automotive systems},
  author={Hernandez, Carles and Abella, Jaume},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={34},
  number={11},
  pages={1718--1729},
  year={2015},
  publisher={IEEE}
}

@article{michalak2005predicting,
  title={Predicting the number of fatal soft errors in Los Alamos National Laboratory's ASC Q supercomputer},
  author={Michalak, Sarah E and Harris, Kevin W and Hengartner, Nicolas W and Takala, Bruce E and Wender, Stephen A},
  journal={IEEE Transactions on Device and Materials Reliability},
  volume={5},
  number={3},
  pages={329--335},
  year={2005},
  publisher={IEEE}
}

@article{snir2014addressing,
  title={Addressing failures in exascale computing},
  author={Snir, Marc and Wisniewski, Robert W and Abraham, Jacob A and Adve, Sarita V and Bagchi, Saurabh and Balaji, Pavan and Belak, Jim and Bose, Pradip and Cappello, Franck and Carlson, Bill and others},
  journal={The International Journal of High Performance Computing Applications},
  volume={28},
  number={2},
  pages={129--173},
  year={2014},
  publisher={Sage Publications Sage UK: London, England}
}


@article{henning2006spec,
  title={SPEC CPU2006 benchmark descriptions},
  author={Henning, John L},
  journal={ACM SIGARCH Computer Architecture News},
  volume={34},
  number={4},
  pages={1--17},
  year={2006},
  publisher={ACM New York, NY, USA}
}

@Misc{NXP_FSBCS,
howpublished = {\url{https://www.nxp.com/docs/en/brochure/SBCAUTOBRA4.pdf}},
title = {{NXP: Functional Safety System Basis Chips (FSSBC)}},
}


@Misc{Linux_5,
howpublished = {\url{https://kernelnewbies.org/Linux_5.7}},
title = {{Linux Kernel 5.7}},
}

@Misc{Xilinx_AXI,
howpublished = {\url{https://www.xilinx.com/products/intellectual-property/axi_interconnect.html}},
title = {{Xilinx: AXI-Interconnect}},
}


@Misc{TSMC_28,
howpublished = {\url{https://www.tsmc.com/english/dedicatedFoundry/technology/logic/l_28nm}},
title = {{28nm PDKs}},
}


@Misc{IBM,
howpublished = {\url{https://www.ibm.com/docs/en/xl-c-and-cpp-aix/16.1?topic=only-overview-constructors-destructors-c
}},
title = {{IBM: Overview of constructors and destructors (C++ only)}},
}

@Misc{Infineon_TriCore,
howpublished = {\url{https://www.infineon.com/cms/en/product/microcontroller/32-bit-tricore-microcontroller/}},
title = {{Infineon: 32-bit TriCore Microcontroller}}
}



@Misc{RenesasRH850,
howpublished = {\url{https://www.renesas.com/eu/en/products/microcontrollers-microprocessors/rh850.html}},
title = {Renesas: RH850 Micro-controller Familiy}
}

@inproceedings{COMET,
author = {Mitropoulou, Konstantina and Porpodas, Vasileios and Jones, Timothy M.},
title = {COMET: communication-optimised multi-threaded error-detection technique},
year = {2016},
isbn = {9781450344821},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2968455.2968508},
doi = {10.1145/2968455.2968508},
abstract = {Relentless technology scaling has made transistors more vulnerable to soft, or transient, errors. To keep systems robust against these, current error detection techniques use different types of redundancy at the hardware or the software level. A consequence of these additional protection mechanisms is that these systems tend to become slower. In particular, software error-detection techniques degrade performance considerably, limiting their uptake.This paper focuses on software redundant multi-threading error detection, a compiler-based technique that makes use of redundant cores within a multi-core system to perform error checking. Implementations of this scheme feature two threads that execute almost the same code: the main thread runs the original code and the checker thread executes code to verify the correctness of the original. The main thread communicates the values that require checking to the checker thread to use in its comparisons.We identify a major performance bottleneck in existing schemes: poorly performing inter-core communication and the generated code associated with it. Our study shows this is a major performance impediment within existing techniques since the two threads require extremely fine-grained communication, on the order of every few instructions. We alleviate this bottleneck with a series of code generation optimisations at the compiler level. We propose COMET (Communication-Optimised Multi-threaded Error-detection Technique), which improves performance across the NAS parallel benchmarks by 31.4\% (on average) compared to the state-of-the-art, without affecting fault-coverage.},
booktitle = {Proceedings of the International Conference on Compilers, Architectures and Synthesis for Embedded Systems},
articleno = {7},
numpages = {10},
keywords = {code generation, communication optimisations, error detection, soft errors},
location = {Pittsburgh, Pennsylvania},
series = {CASES '16}
}

@inproceedings{batcher1999instruction,
  title={Instruction randomization self test for processor cores},
  author={Batcher, Ken and Papachristou, Christos},
  booktitle={Proceedings 17th IEEE VLSI Test Symposium (Cat. No. PR00146)},
  pages={34--40},
  year={1999},
  organization={IEEE}
}

@article{bernardi2015development,
  title={Development flow for on-line core self-test of automotive microcontrollers},
  author={Bernardi, Paolo and Cantoro, Riccardo and De Luca, Sergio and S{\'a}nchez, Ernesto and Sansonetti, Alessandro},
  journal={IEEE Transactions on Computers},
  volume={65},
  number={3},
  pages={744--754},
  year={2015},
  publisher={IEEE}
}
@inproceedings{rotenberg1999ar,
  title={AR-SMT: A microarchitectural approach to fault tolerance in microprocessors},
  author={Rotenberg, Eric},
  booktitle={Digest of Papers. Twenty-Ninth Annual International Symposium on Fault-Tolerant Computing (Cat. No. 99CB36352)},
  pages={84--91},
  year={1999},
  organization={IEEE}
}

@article{mukherjee2002detailed,
  title={Detailed design and evaluation of redundant multithreading alternatives},
  author={Mukherjee, Shubhendu S and Kontz, Michael and Reinhardt, Steven K},
  journal={ACM SIGARCH Computer Architecture News},
  volume={30},
  number={2},
  pages={99--110},
  year={2002},
  publisher={ACM New York, NY, USA}
}


@inproceedings{reinhardt2000transient,
  title={Transient fault detection via simultaneous multithreading},
  author={Reinhardt, Steven K and Mukherjee, Shubhendu S},
  booktitle={Proceedings of the 27th annual international symposium on Computer architecture},
  pages={25--36},
  year={2000}
}

@article{feero2008networks,
  title={Networks-on-chip in a three-dimensional environment: A performance evaluation},
  author={Feero, Brett Stanley and Pande, Partha Pratim},
  journal={IEEE Transactions on computers},
  volume={58},
  number={1},
  pages={32--45},
  year={2008},
  publisher={IEEE}
}


@article{doweck2017inside,
  title={Inside 6th-generation intel core: New microarchitecture code-named skylake},
  author={Doweck, Jack and Kao, Wen-Fu and Lu, Allen Kuan-yu and Mandelblat, Julius and Rahatekar, Anirudha and Rappoport, Lihu and Rotem, Efraim and Yasin, Ahmad and Yoaz, Adi},
  journal={IEEE Micro},
  volume={37},
  number={2},
  pages={52--62},
  year={2017},
  publisher={IEEE}
}

@article{de2018lockstep,
  title={Lockstep dual-core ARM A9: Implementation and resilience analysis under heavy ion-induced soft errors},
  author={de Oliveira, {\'A}dria Barros and Rodrigues, Gennaro Severino and Kastensmidt, Fernanda Lima and Added, Nemitala and Macchione, Eduardo LA and Aguiar, Vitor AP and Medina, Nilberto H and Silveira, Marcilei AG},
  journal={IEEE Transactions on Nuclear Science},
  volume={65},
  number={8},
  pages={1783--1790},
  year={2018},
  publisher={IEEE}
}


@article{iso201126262,
  title={26262: Road vehicles-Functional safety},
  author={ISO, ISO26262},
  year={2018}
}

@book{rierson2017developing,
  title={Developing safety-critical software: a practical guide for aviation software and DO-178C compliance},
  author={Rierson, Leanna},
  year={2017},
  publisher={CRC Press}
}


@inproceedings{austin1999diva,
  title={DIVA: A reliable substrate for deep submicron microarchitecture design},
  author={Austin, Todd M},
  booktitle={MICRO-32. Proceedings of the 32nd Annual ACM/IEEE International Symposium on Microarchitecture},
  pages={196--207},
  year={1999},
  organization={IEEE}
}

@article{barney2009posix,
  title={POSIX threads programming},
  author={Barney, Blaise},
  journal={National Laboratory. Dispon{\'\i}vel em:< https://computing. llnl. gov/tutorials/pthreads/> Acesso em},
  volume={5},
  pages={46},
  year={2009}
}




@inproceedings{iturbe2016triple,
  title={A triple core lock-step (tcls) arm{\textregistered} cortex{\textregistered}-r5 processor for safety-critical and ultra-reliable applications},
  author={Iturbe, Xabier and Venu, Balaji and Ozer, Emre and Das, Shidhartha},
  booktitle={2016 46th Annual IEEE/IFIP International Conference on Dependable Systems and Networks Workshop (DSN-W)},
  pages={246--249},
  year={2016},
  organization={IEEE}
}

@article{iturbe2019arm,
  title={The Arm triple core lock-step (TCLS) processor},
  author={Iturbe, Xabier and Venu, Balaji and Ozer, Emre and Poupat, Jean-Luc and Gimenez, Gregoire and Zurek, Hans-Ulrich},
  journal={ACM Transactions on Computer Systems (TOCS)},
  volume={36},
  number={3},
  pages={1--30},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{ainsworth2018parallel,
  title={Parallel error detection using heterogeneous cores},
  author={Ainsworth, Sam and Jones, Timothy M},
  booktitle={2018 48th Annual IEEE/IFIP International Conference on Dependable Systems and Networks (DSN)},
  pages={338--349},
  year={2018},
  organization={IEEE}
}

@inproceedings{ainsworth2019paramedic,
  title={Paramedic: Heterogeneous parallel error correction},
  author={Ainsworth, Sam and Jones, Timothy M},
  booktitle={2019 49th Annual IEEE/IFIP International Conference on Dependable Systems and Networks (DSN)},
  pages={201--213},
  year={2019},
  organization={IEEE}
}

@inproceedings{ainsworth2021paradox,
  title={Paradox: Eliminating voltage margins via heterogeneous fault tolerance},
  author={Ainsworth, Sam and Zoubritzky, Lionel and Mycroft, Alan and Jones, Timothy M},
  booktitle={2021 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={520--532},
  year={2021},
  organization={IEEE}
}

@article{zeinolabedin2020real,
  title={Real-time hardware implementation of arm coresight trace decoder},
  author={Zeinolabedin, Seyed Mohammad Ali and Partzsch, Johannes and Mayr, Christian},
  journal={IEEE Design \& Test},
  volume={38},
  number={1},
  pages={69--77},
  year={2020},
  publisher={IEEE}
}

@inproceedings{kuzhiyelil2020towards,
  title={Towards transparent control-flow integrity in safety-critical systems},
  author={Kuzhiyelil, Don and Zieris, Philipp and Kadar, Marine and Tverdyshev, Sergey and Fohler, Gerhard},
  booktitle={International Conference on Information Security},
  pages={290--311},
  year={2020},
  organization={Springer}
}

@article{ge2017griffin,
  title={Griffin: Guarding control flows using intel processor trace},
  author={Ge, Xinyang and Cui, Weidong and Jaeger, Trent},
  journal={ACM SIGPLAN Notices},
  volume={52},
  number={4},
  pages={585--598},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@inproceedings{deng2010flexible,
  title={Flexible and efficient instruction-grained run-time monitoring using on-chip reconfigurable fabric},
  author={Deng, Daniel Y and Lo, Daniel and Malysa, Greg and Schneider, Skyler and Suh, G Edward},
  booktitle={2010 43rd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={137--148},
  year={2010},
  organization={IEEE}
}

@article{chen2008flexible,
  title={Flexible hardware acceleration for instruction-grain program monitoring},
  author={Chen, Shimin and Kozuch, Michael and Strigkos, Theodoros and Falsafi, Babak and Gibbons, Phillip B and Mowry, Todd C and Ramachandran, Vijaya and Ruwase, Olatunji and Ryan, Michael and Vlachos, Evangelos},
  journal={ACM SIGARCH Computer Architecture News},
  volume={36},
  number={3},
  pages={377--388},
  year={2008},
  publisher={ACM New York, NY, USA}
}
@inproceedings{fytraki2014fade,
  title={FADE: A programmable filtering accelerator for instruction-grain monitoring},
  author={Fytraki, Sotiria and Vlachos, Evangelos and Kocberber, Onur and Falsafi, Babak and Grot, Boris},
  booktitle={2014 IEEE 20th International Symposium on High Performance Computer Architecture (HPCA)},
  pages={108--119},
  year={2014},
  organization={IEEE}
}

@inproceedings{chen2021herqules,
  title={HerQules: Securing programs via hardware-enforced message queues},
  author={Chen, Daming D and Lim, Wen Shih and Bakhshalipour, Mohammad and Gibbons, Phillip B and Hoe, James C and Parno, Bryan},
  booktitle={Proceedings of the 26th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={773--788},
  year={2021}
}



@inproceedings{demme2013feasibility,
  title={On the feasibility of online malware detection with performance counters},
  author={Demme, John and Maycock, Matthew and Schmitz, Jared and Tang, Adrian and Waksman, Adam and Sethumadhavan, Simha and Stolfo, Salvatore},
  journal={ACM SIGARCH computer architecture news},
  volume={41},
  number={3},
  pages={559--570},
  year={2013},
  publisher={ACM New York, NY, USA}
}

@inproceedings{milenkovic2005hardware,
  title={Hardware support for code integrity in embedded processors},
  author={Milenkovi{\'c}, Milena and Milenkovi{\'c}, Aleksandar and Jovanov, Emil},
  booktitle={Proceedings of the 2005 international conference on Compilers, architectures and synthesis for embedded systems},
  pages={55--65},
  year={2005}
}


@inproceedings{papazian2020new,
  title={New 3rd Gen Intel{\textregistered} Xeon{\textregistered} Scalable Processor (Codename: Ice Lake-SP)},
  author={Papazian, Irma Esmer},
  booktitle={Hot Chips Symposium},
  year={2020}
}

@inproceedings{nyman2017hardscope,
  title={Hardscope: Thwarting DOP with hardware-assisted run-time scope enforcement},
  author={Nyman, Thomas and Dessouky, Ghada and Zeitouni, Shaza and Lehikoinen, Aaro and Paverd, Andrew and Asokan, N and Sadeghi, Ahmad-Reza},
  journal={arXiv preprint arXiv:1705.10295},
  year={2017}
}

@article{woodruff2014cheri,
  title={The CHERI capability model: Revisiting RISC in an age of risk},
  author={Woodruff, Jonathan and Watson, Robert NM and Chisnall, David and Moore, Simon W and Anderson, Jonathan and Davis, Brooks and Laurie, Ben and Neumann, Peter G and Norton, Robert and Roe, Michael},
  journal={ACM SIGARCH Computer Architecture News},
  volume={42},
  number={3},
  pages={457--468},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{xia2019cherivoke,
  title={Cherivoke: Characterising pointer revocation using cheri capabilities for temporal memory safety},
  author={Xia, Hongyan and Woodruff, Jonathan and Ainsworth, Sam and Filardo, Nathaniel W and Roe, Michael and Richardson, Alexander and Rugg, Peter and Neumann, Peter G and Moore, Simon W and Watson, Robert NM and others},
  booktitle={Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={545--557},
  year={2019}
}

@inproceedings{devietti2008hardbound,
  title={Hardbound: Architectural support for spatial safety of the C programming language},
  author={Devietti, Joe and Blundell, Colin and Martin, Milo MK and Zdancewic, Steve},
  journal={ACM SIGOPS Operating Systems Review},
  volume={42},
  number={2},
  pages={103--114},
  year={2008},
  publisher={ACM New York, NY, USA}
}

@inproceedings{bannister2019memory,
  title={Memory Tagging Extension},
  author={Bannister, Steve},
  journal={ARM},
  year={2019}
}

@inproceedings{celio2019broom,
  title={Broom: an open-source out-of-order processor with resilient low-voltage operation in 28-nm cmos},
  author={Celio, Christopher and Chiu, Pi-Feng and Asanovi{\'c}, Krste and Nikoli{\'c}, Borivoje and Patterson, David},
  journal={IEEE Micro},
  volume={39},
  number={2},
  pages={52--60},
  year={2019},
  publisher={IEEE}
}

@inproceedings{davidson2018celerity,
  title={The Celerity open-source 511-core RISC-V tiered accelerator fabric: Fast architectures and design methodologies for fast chips},
  author={Davidson, Scott and Xie, Shaolin and Torng, Christopher and Al-Hawai, Khalid and Rovinski, Austin and Ajayi, Tutu and Vega, Luis and Zhao, Chun and Zhao, Ritchie and Dai, Steve and others},
  journal={IEEE Micro},
  volume={38},
  number={2},
  pages={30--41},
  year={2018},
  publisher={IEEE}
}


@mastersthesis{Pala2017rocc,
  title={Design and programming of a coprocessor for a RISC-V architecture},
  author={Davide, Pala},
  year={2017},
  school={Politecnico di Torino}
}

@inproceedings{bienia2008parsec,
  title={The PARSEC benchmark suite: Characterization and architectural implications},
  author={Bienia, Christian and Kumar, Sanjeev and Singh, Jaswinder Pal and Li, Kai},
  booktitle={Proceedings of the 17th international conference on Parallel architectures and compilation techniques},
  pages={72--81},
  year={2008}
}


@inproceedings{erdHos2022minesweeper,
  title={MineSweeper: a “clean sweep” for drop-in use-after-free prevention},
  author={Erd{\H{o}}s, M{\'a}rton and Ainsworth, Sam and Jones, Timothy M},
  booktitle={Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={212--225},
  year={2022}
}



@article{holly2005reusable,
  title={A reusable Duff device},
  author={Holly, Ralf},
  journal={Dr. Dobb's Journal},
  volume={30},
  number={8},
  pages={73--74},
  year={2005}
}

@inproceedings{dangsan,
  title={Dangsan: Scalable use-after-free detection},
  author={Van Der Kouwe, Erik and Nigade, Vinod and Giuffrida, Cristiano},
  booktitle={Proceedings of the Twelfth European Conference on Computer Systems},
  pages={405--419},
  year={2017}
}

@inproceedings{verma2007understanding,
  title={Understanding clock domain crossing issues},
  author={Verma, Saurabh and Dabare, Ashima S},
  journal={EE Times},
  year={2007}
}

@misc{duff1988duff,
  title={Duff’s device},
  author={Duff, Tom},
  year={1988}
}

@book{gajski1996principles,
  title={Principles of digital design},
  author={Gajski, Daniel D},
  year={1996},
  publisher={Prentice-Hall, Inc.}
}

@inproceedings{wagner2017diasys,
  title={DiaSys: Improving SoC insight through on-chip diagnosis},
  author={Wagner, Philipp and Wild, Thomas and Herkersdorf, Andreas},
  journal={Journal of Systems Architecture},
  volume={75},
  pages={120--132},
  year={2017},
  publisher={Elsevier}
}


@inproceedings{khasawneh2015ensemble,
  title={Ensemble learning for low-level hardware-supported malware detection},
  author={Khasawneh, Khaled N and Ozsoy, Meltem and Donovick, Caleb and Abu-Ghazaleh, Nael and Ponomarev, Dmitry},
  booktitle={Research in Attacks, Intrusions, and Defenses: 18th International Symposium, RAID 2015, Kyoto, Japan, November 2-4, 2015. Proceedings},
  pages={3--25},
  year={2015},
  organization={Springer}
}



@inproceedings{jiang2020pythia,
  title={Pythia-mcs: Enabling quarter-clairvoyance in i/o-driven mixed-criticality systems},
  author={Jiang, Zhe and Yang, Kecheng and Fisher, Nathan and Audsley, Neil and Dong, Zheng},
  booktitle={2020 IEEE Real-Time Systems Symposium (RTSS)},
  pages={38--50},
  year={2020},
  organization={IEEE}
}

@inproceedings{binkert2011gem5,
  title={The gem5 simulator},
  author={Binkert, Nathan and Beckmann, Bradford and Black, Gabriel and Reinhardt, Steven K and Saidi, Ali and Basu, Arkaprava and Hestness, Joel and Hower, Derek R and Krishna, Tushar and Sardashti, Somayeh and others},
  journal={ACM SIGARCH computer architecture news},
  volume={39},
  number={2},
  pages={1--7},
  year={2011},
  publisher={ACM New York, NY, USA}
}



@inproceedings{shetty2006heapmon,
  title={Heapmon: A helper-thread approach to programmable, automatic, and low-overhead memory bug detection},
  author={Shetty, Rithin and Kharbutli, Mazen and Solihin, Yan and Prvulovic, Milos},
  journal={IBM Journal of Research and Development},
  volume={50},
  number={2.3},
  pages={261--275},
  year={2006},
  publisher={IBM}
}

@inproceedings{lo2015run,
  title={Run-time monitoring with adjustable overhead using dataflow-guided filtering},
  author={Lo, Daniel and Chen, Tao and Ismail, Mohamed and Suh, G Edward},
  booktitle={2015 IEEE 21st International Symposium on High Performance Computer Architecture (HPCA)},
  pages={662--674},
  year={2015},
  organization={IEEE}
}

@inproceedings{corliss2003dise,
  title={DISE: A programmable macro engine for customizing applications},
  author={Corliss, Marc L and others},
  journal={ACM SIGARCH Computer Architecture News},
  year={2003}
}

@inproceedings{francillon2009defending,
  title={Defending embedded systems against control flow attacks},
  author={Francillon, Aur{\'e}lien and Perito, Daniele and Castelluccia, Claude},
  booktitle={Proceedings of the first ACM workshop on Secure execution of untrusted code},
  pages={19--26},
  year={2009}
}

@inproceedings{kim2014architectural,
  title={Architectural support for mitigating row hammering in DRAM memories},
  author={Kim, Dae-Hyun and Nair, Prashant J and Qureshi, Moinuddin K},
  journal={IEEE Computer Architecture Letters},
  volume={14},
  number={1},
  pages={9--12},
  year={2014},
  publisher={IEEE}
}

@inproceedings{ozsoy2015malware,
  title={Malware-aware processors: A framework for efficient online malware detection},
  author={Ozsoy, Meltem and Donovick, Caleb and Gorelik, Iakov and Abu-Ghazaleh, Nael and Ponomarev, Dmitry},
  booktitle={2015 IEEE 21st International Symposium on High Performance Computer Architecture (HPCA)},
  pages={651--661},
  year={2015},
  organization={IEEE}
}

@inproceedings{wehbe2018hardware,
  title={Hardware-based run-time code integrity in embedded devices},
  author={Wehbe, Taimour and Mooney, Vincent and Keezer, David},
  journal={Cryptography},
  volume={2},
  number={3},
  pages={20},
  year={2018},
  publisher={MDPI}
}

@inproceedings{davi2015hafix,
  title={HAFIX: Hardware-assisted flow integrity extension},
  author={Davi, Lucas and Hanreich, Matthias and Paul, Debayan and Sadeghi, Ahmad-Reza and Koeberl, Patrick and Sullivan, Dean and Arias, Orlando and Jin, Yier},
  booktitle={Proceedings of the 52nd Annual Design Automation Conference},
  pages={1--6},
  year={2015}
}

@inproceedings{zhang2011homealone,
  title={Homealone: Co-residency detection in the cloud via side-channel analysis},
  author={Zhang, Yinqian and Juels, Ari and Oprea, Alina and Reiter, Michael K},
  booktitle={2011 IEEE symposium on security and privacy},
  pages={313--328},
  year={2011},
  organization={IEEE}
}


@inproceedings{szekeres2013sok,
  title={Sok: Eternal war in memory},
  author={Szekeres, Laszlo and Payer, Mathias and Wei, Tao and Song, Dawn},
  booktitle={2013 IEEE Symposium on Security and Privacy},
  pages={48--62},
  year={2013},
  organization={IEEE}
}

@inproceedings{zhang2015control,
  title={Control flow and code integrity for COTS binaries: An effective defense against real-world ROP attacks},
  author={Zhang, Mingwei and Sekar, R},
  booktitle={Proceedings of the 31st Annual Computer Security Applications Conference},
  pages={91--100},
  year={2015}
}

@inproceedings{checkoway2010return,
  title={Return-oriented programming without returns},
  author={Checkoway, Stephen and Davi, Lucas and Dmitrienko, Alexandra and Sadeghi, Ahmad-Reza and Shacham, Hovav and Winandy, Marcel},
  booktitle={Proceedings of the 17th ACM conference on Computer and communications security},
  pages={559--572},
  year={2010}
}

@inproceedings{erlingsson2000irm,
  title={IRM enforcement of Java stack inspection},
  author={Erlingsson, Ulfar and Schneider, Fred B},
  booktitle={Proceeding 2000 IEEE Symposium on Security and Privacy. S\&P 2000},
  pages={246--255},
  year={2000},
  organization={IEEE}
}

@inproceedings{ghosal2022secure,
  title={Secure over-the-air software update for connected vehicles},
  author={Ghosal, Amrita and Halder, Subir and Conti, Mauro},
  journal={Computer Networks},
  volume={218},
  pages={109394},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{serebryany2012addresssanitizer,
  title={$\{$AddressSanitizer$\}$: A fast address sanity checker},
  author={Serebryany, Konstantin and Bruening, Derek and Potapenko, Alexander and Vyukov, Dmitriy},
  booktitle={2012 USENIX annual technical conference (USENIX ATC 12)},
  pages={309--318},
  year={2012}
}

@inproceedings{necula2002ccured,
  title={CCured: Type-safe retrofitting of legacy code},
  author={Necula, George C and McPeak, Scott and Weimer, Westley},
  booktitle={Proceedings of the 29th ACM SIGPLAN-SIGACT symposium on Principles of programming languages},
  pages={128--139},
  year={2002}
}

@inproceedings{cowan2000buffer,
  title={Buffer overflows: Attacks and defenses for the vulnerability of the decade},
  author={Cowan, Crispin and Wagle, F and Pu, Calton and Beattie, Steve and Walpole, Jonathan},
  booktitle={Proceedings DARPA Information Survivability Conference and Exposition. DISCEX'00},
  volume={2},
  pages={119--129},
  year={2000},
  organization={IEEE}
}

@article{abadi2009control,
  title={Control-flow integrity principles, implementations, and applications},
  author={Abadi, Mart{\'\i}n and Budiu, Mihai and Erlingsson, Ulfar and Ligatti, Jay},
  journal={ACM Transactions on Information and System Security (TISSEC)},
  volume={13},
  number={1},
  pages={1--40},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@inproceedings{austin1994efficient,
  title={Efficient detection of all pointer and array access errors},
  author={Austin, Todd M and Breach, Scott E and Sohi, Gurindar S},
  booktitle={Proceedings of the ACM SIGPLAN 1994 conference on Programming Language Design and Implementation},
  pages={290--301},
  year={1994}
}

@inproceedings{jiang2018bluevisor,
  title={Bluevisor: A scalable real-time hardware hypervisor for many-core embedded systems},
  author={Jiang, Zhe and Audsley, Neil C and Dong, Pan},
  booktitle={2018 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS)},
  pages={75--84},
  year={2018},
  organization={IEEE}
}

@inproceedings{becher2011mobile,
  title={Mobile security catching up? revealing the nuts and bolts of the security of mobile devices},
  author={Becher, Michael and Freiling, Felix C and Hoffmann, Johannes and Holz, Thorsten and Uellenbeck, Sebastian and Wolf, Christopher},
  booktitle={2011 IEEE Symposium on Security and Privacy},
  pages={96--111},
  year={2011},
  organization={IEEE}
}

@inproceedings{zhou2012dissecting,
  title={Dissecting android malware: Characterization and evolution},
  author={Zhou, Yajin and Jiang, Xuxian},
  booktitle={2012 IEEE symposium on security and privacy},
  pages={95--109},
  year={2012},
  organization={IEEE}
}

@inproceedings{felt2011android,
  title={Android permissions demystified},
  author={Felt, Adrienne Porter and Chin, Erika and Hanna, Steve and Song, Dawn and Wagner, David},
  booktitle={Proceedings of the 18th ACM conference on Computer and communications security},
  pages={627--638},
  year={2011}
}

@Misc{Oracle2016,
  title={Oracle’s SPARC T7 and SPARC M7 Server Architecture},
  author={Oracle},
  year={2016}
}




@inproceedings{BTI,
booktitle = {\url{hhttps://developer.arm.com/documentation/100748/latest/Security-features-supported-in-Arm-Compiler-for-Embedded/}},
author = {{ARM BTI}},
year={2023}
}


@inproceedings{shanbhogue2019security,
  title={Security analysis of processor instruction set architecture for enforcing control-flow integrity},
  author={Shanbhogue, Vedvyas and Gupta, Deepak and Sahita, Ravi},
  booktitle={Proceedings of the 8th International Workshop on Hardware and Architectural Support for Security and Privacy},
  pages={1--11},
  year={2019}
}

@Misc{x2,
howpublished = {\url{https://developer.arm.com/documentation/101803/0200/The-Cortex-X2--core}},
author = {{ARM Cortex-X2}}
}

@Misc{a710,
howpublished = {\url{https://www.arm.com/products/silicon-ip-cpu/cortex-a/cortex-a710}},
author = {{ARM Cortex-A710}}
}

@Misc{a510,
howpublished = {\url{https://www.arm.com/products/silicon-ip-cpu/cortex-a/cortex-a510}},
author = {{ARM Cortex-A510}}
}

@Misc{coresight,
howpublished = {\url{https://developer.arm.com/Architectures/CoreSight\%20Architecture}},
author = {{ARM Cortex-Sight}}
}

@article{guide2011intel,
  title={Intel{\textregistered} 64 and ia-32 architectures software developer’s manual},
  author={Guide, Part},
  journal={Volume 3B: System programming Guide, Part},
  volume={2},
  number={11},
  pages={1--64},
  year={2011}
}

@Misc{9000,
howpublished = {\url{https://www.mediatek.com/products/smartphones-2/mediatek-dimensity-9000plus}},
author = {{MediaTek Dimensity 9000}}
}

@Misc{LAM,
howpublished = {\url{https://lpc.events/event/11/contributions/LAM-LPC-2021.pdf}},
author = {{Intel LAM}},
year = {2021}
}

@inproceedings{zhang2018hcic,
  title={HCIC: Hardware-assisted control-flow integrity checking},
  author={Zhang, Jiliang and Qi, Binhang and Qin, Zheng and Qu, Gang},
  journal={IEEE Internet of Things Journal},
  
  year={2018},
  publisher={IEEE}
}

@inproceedings{christoulakis2016hcfi,
  title={HCFI: Hardware-enforced control-flow integrity},
  author={Christoulakis, Nick and Christou, George and Athanasopoulos, Elias and Ioannidis, Sotiris},
  booktitle={Proceedings of the Sixth ACM Conference on Data and Application Security and Privacy},
  pages={38--49},
  year={2016}
}


@inproceedings{CET,
howpublished = {\url{https://www.intel.com/content/dam/develop/external/us/en/documents/catc17-introduction-intel-cet-844137.pdf}},
author = {{Intel CET}},
year = {2023}
}

@inproceedings{vera2020inside,
  title={Inside Tiger Lake: Intel's Next Generation Mobile Client CPU},
  author={Vera, Xavier},
  booktitle={Hot Chips Symposium},
  year={2020}
}

@inproceedings{restuccia2020axi,
  title={Axi hyperconnect: A predictable, hypervisor-level interconnect for hardware accelerators in fpga soc},
  author={Restuccia, Francesco and Biondi, Alessandro and Marinoni, Mauro and Cicero, Giorgiomaria and Buttazzo, Giorgio},
  booktitle={2020 57th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@Misc{armtracer,
howpublished = {\url{https://boom-core.org/docs/HC30.Berkeley.Celio-Chiu.final.pdf}},
author = {Celio, Christopher and Chiu, Pi-Feng and Asanovic, Krste and Patterson, David and Nikolic, Borivoje},
booktitle={Hot Chips},
year = {2018}
}


@Misc{rboom,
howpublished = {\url{https://developer.arm.com/documentation/102520/0100/}},
author = {ARM}
}

@article{jiang2022axi,
  title={AXI-IC$^\text{RT}$: Towards a Real-Time AXI-Interconnect for Highly Integrated SoCs},
  author={Jiang, Zhe and Yang, Kecheng and Fisher, Nathan and Gray, Ian and Audsley, Neil C and Dong, Zheng},
  journal={IEEE Transactions on Computers},
  volume={72},
  number={3},
  pages={786--799},
  year={2022},
  publisher={IEEE}
}


@Misc{riscvcompare,
howpublished = {\url{https://www.esperanto.ai/wp-content/uploads/2018/12/Esperanto-Maxes-Out-RISC-V.pdf}},
author = {The Linely Group}
}

@Misc{sparcadi,
howpublished = {\url{https://docs.oracle.com/cd/E53394_01/html/E54815/gqajs.html}},
author = {Sparc ADI support}
}




@inproceedings{zecar,
howpublished = {\url{https://zecar.com/reviews/byd-atto-3-more-details-revealed-apple-carplay-android-auto-coming-in-q3-2022}},
author = {Zecar},
year = {2023}
}

@inproceedings{ss_llvm,
howpublished = {\url{https://clang.llvm.org/docs/ShadowCallStack.html}},
author = {LLVM},
year = {2023}
}


@inproceedings{checkoway2011comprehensive,
  title={Comprehensive experimental analyses of automotive attack surfaces},
  author={Checkoway, Stephen and McCoy, Damon and Kantor, Brian and Anderson, Danny and Shacham, Hovav and Savage, Stefan and Koscher, Karl and Czeskis, Alexei and Roesner, Franziska and Kohno, Tadayoshi},
  booktitle={20th USENIX security symposium (USENIX Security 11)},
  year={2011}
}

@inproceedings{van2020lvi,
  title={LVI: Hijacking transient execution through microarchitectural load value injection},
  author={Van Bulck, Jo and Moghimi, Daniel and Schwarz, Michael and Lippi, Moritz and Minkin, Marina and Genkin, Daniel and Yarom, Yuval and Sunar, Berk and Gruss, Daniel and Piessens, Frank},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={54--72},
  year={2020},
  organization={IEEE}
}


@inproceedings{weisse2018foreshadow,
  title={Foreshadow-NG: Breaking the virtual memory abstraction with transient out-of-order execution},
  author={Weisse, Ofir and Van Bulck, Jo and Minkin, Marina and Genkin, Daniel and Kasikci, Baris and Piessens, Frank and Silberstein, Mark and Strackx, Raoul and Wenisch, Thomas F and Yarom, Yuval},
  year={2018},
      booktitle = {Proceedings of the 27th {USENIX} Security Symposium}
}

@inproceedings{chen2010side,
  title={Side-channel leaks in web applications: A reality today, a challenge tomorrow},
  author={Chen, Shuo and Wang, Rui and Wang, XiaoFeng and Zhang, Kehuan},
  booktitle={2010 IEEE Symposium on Security and Privacy},
  pages={191--206},
  year={2010},
  organization={IEEE}
}

@inproceedings{arthur2015locking,
  title={Locking down insecure indirection with hardware-based control-data isolation},
  author={Arthur, William and Madeka, Sahil and Das, Reetuparna and Austin, Todd},
  booktitle={Proceedings of the 48th International Symposium on Microarchitecture},
  pages={115--127},
  year={2015}
}

@inproceedings{sabt2015trusted,
  title={Trusted execution environment: what it is, and what it is not},
  author={Sabt, Mohamed and Achemlal, Mohammed and Bouabdallah, Abdelmadjid},
  booktitle={2015 IEEE Trustcom/BigDataSE/Ispa},
  volume={1},
  pages={57--64},
  year={2015},
  organization={IEEE}
}

@inproceedings{ristenpart2009hey,
  title={Hey, you, get off of my cloud: exploring information leakage in third-party compute clouds},
  author={Ristenpart, Thomas and Tromer, Eran and Shacham, Hovav and Savage, Stefan},
  booktitle={Proceedings of the 16th ACM conference on Computer and communications security},
  pages={199--212},
  year={2009}
}

@inproceedings{oren2015spy,
  title={The spy in the sandbox: Practical cache attacks in javascript and their implications},
  author={Oren, Yossef and Kemerlis, Vasileios P and Sethumadhavan, Simha and Keromytis, Angelos D},
  booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
  pages={1406--1418},
  year={2015}
}


@inproceedings{waldrop2016chips,
  title={The chips are down for Moore’s law},
  author={Waldrop, M Mitchell},
  journal={Nature News},
  volume={530},
  number={7589},
  pages={144},
  year={2016}
}

@inproceedings{hennessy2019new,
  title={A new golden age for computer architecture},
  author={Hennessy, John L and Patterson, David A},
  journal={Communications of the ACM},
  volume={62},
  number={2},
  pages={48--60},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{xavier2013performance,
  title={Performance evaluation of container-based virtualization for high performance computing environments},
  author={Xavier, Miguel G and Neves, Marcelo V and Rossi, Fabio D and Ferreto, Tiago C and Lange, Timoteo and De Rose, Cesar AF},
  booktitle={2013 21st Euromicro International Conference on Parallel, Distributed, and Network-Based Processing},
  pages={233--240},
  year={2013},
  organization={IEEE}
}

@inproceedings{garraghan2013analysis,
  title={An analysis of the server characteristics and resource utilization in google cloud},
  author={Garraghan, Peter and Townend, Paul and Xu, Jie},
  booktitle={2013 IEEE International Conference on Cloud Engineering (IC2E)},
  pages={124--131},
  year={2013},
  organization={IEEE}
}

@book{fuller2011future,
  title={The future of computing performance: game over or next level?},
  author={Fuller, Samuel H and Millett, Lynette I},
  year={2011},
  publisher={National Academy Press}
}

@inproceedings{buyya2009cloud,
  title={Cloud computing and emerging IT platforms: Vision, hype, and reality for delivering computing as the 5th utility},
  author={Buyya, Rajkumar and Yeo, Chee Shin and Venugopal, Srikumar and Broberg, James and Brandic, Ivona},
  journal={Future Generation computer systems},
  volume={25},
  number={6},
  pages={599--616},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{cerdeira2020sok,
  title={Sok: Understanding the prevailing security vulnerabilities in trustzone-assisted tee systems},
  author={Cerdeira, David and Santos, Nuno and Fonseca, Pedro and Pinto, Sandro},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={1416--1432},
  year={2020},
  organization={IEEE}
}

@inproceedings{burns2017survey,
  title={A survey of research into mixed criticality systems},
  author={Burns, Alan and Davis, Robert I},
  journal={ACM Computing Surveys (CSUR)},
  volume={50},
  number={6},
  pages={1--37},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@inproceedings{brenner2017trapps,
  title={TrApps: Secure compartments in the evil cloud},
  author={Brenner, Stefan and Goltzsche, David and Kapitza, R{\"u}diger},
  booktitle={Proceedings of the 1st International Workshop on Security and Dependability of Multi-Domain Infrastructures},
  pages={1--6},
  year={2017}
}

@inproceedings{restuccia2022bounding,
  title={Bounding Memory Access Times in Multi-Accelerator Architectures on FPGA SoCs},
  author={Restuccia, Francesco and Pagani, Marco and Biondi, Alessandro and Marinoni, Mauro and Buttazzo, Giorgio},
  journal={IEEE Transactions on Computers},
  volume={72},
  number={1},
  pages={154--167},
  year={2022},
  publisher={IEEE}
}

@inproceedings{damian2022scaie,
  title={SCAIE-V: an open-source SCAlable interface for ISA extensions for RISC-V processors},
  author={Damian, Mihaela and Oppermann, Julian and Spang, Christoph and Koch, Andreas},
  booktitle={Proceedings of the 59th ACM/IEEE Design Automation Conference},
  pages={169--174},
  year={2022}
}


@inproceedings{jiang2022bluescale,
  title={BlueScale: a scalable memory architecture for predictable real-time computing on highly integrated SoCs},
  author={Jiang, Zhe and Yang, Kecheng and Audsley, Neil and Fisher, Nathan and Shi, Weisong and Dong, Zheng},
  booktitle={Proceedings of the 59th ACM/IEEE Design Automation Conference},
  pages={1261--1266},
  year={2022}
}

@inproceedings{ainsworth2020guardian,
  title={The guardian council: Parallel programmable hardware security},
  author={Ainsworth, Sam and Jones, Timothy M},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={1277--1293},
  year={2020}
}

@inproceedings{zhao2020sonicboom,
  title={Sonicboom: The 3rd generation berkeley out-of-order machine},
  author={Zhao, Jerry and Korpan, Ben and Gonzalez, Abraham and Asanovic, Krste},
  booktitle={Fourth Workshop on Computer Architecture Research with RISC-V},
  volume={5},
  pages={1--7},
  year={2020}
}

@article{asanovic2016rocket,
  title={The rocket chip generator},
  author={Asanovic, Krste and Avizienis, Rimas and Bachrach, Jonathan and Beamer, Scott and Biancolin, David and Celio, Christopher and Cook, Henry and Dabbelt, Daniel and Hauser, John and Izraelevitz, Adam and others},
  journal={EECS Department, University of California, Berkeley, Tech. Rep. UCB/EECS-2016-17},
  volume={4},
  pages={6--2},
  year={2016}
}

@inproceedings{karandikar2018firesim,
  title={FireSim: FPGA-accelerated cycle-exact scale-out system simulation in the public cloud},
  author={Karandikar, Sagar and Mao, Howard and Kim, Donggyu and Biancolin, David and Amid, Alon and Lee, Dayeol and Pemberton, Nathan and Amaro, Emmanuel and Schmidt, Colin and Chopra, Aditya and others},
  booktitle={2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)},
  pages={29--42},
  year={2018},
  organization={IEEE}
}


@inproceedings{m1pro-overview,
  title={Apple M1 Pro Die Shot},
  booktitle={\url{https://www.anandtech.com/show/17019/apple-announced-m1-pro-m1-max-giant-new-socs-with-allout-performance}},
  year={2021}
}

@inproceedings{m1pro-micro,
  title={Firestorm Pipeline Overview},
  author={Dougall Johnson},
  booktitle={\url{https://dougallj.github.io/applecpu/firestorm.html}},
  year={2022}
}

@inproceedings{a76-overview,
  title={Kirin 980 Die Shot},
  booktitle={\url{https://www.anandtech.com/show/13564/chiprebel-releases-kirin-980-die-shot-cortex-a76s-mali-g76-in-view}},
  year={2018}
}

@inproceedings{a76-arch,
  title={Cortex-A76},
  author={ARM},
  booktitle={\url{https://developer.arm.com/Processors/Cortex-A76}},
  year={2018}
}


@inproceedings{big-little,
  title={big.LITTLE Architecture},
  author={ARM},
  booktitle={\url{https://www.arm.com/technologies/big-little}},
  year={2024}
}

@inproceedings{alderlake-micro,
  title={Alder Lake: Microarchitecture},
  author={Intel},
  booktitle={\url{https://en.wikichip.org/wiki/intel/microarchitectures/alder\_lake}},
  year={2022}
}

@inproceedings{alderlake-spec,
  title={Alder Lake: Specification},
  author={Intel},
  booktitle={\url{https://www.intel.co.uk/content/www/uk/en/products/platforms/details/alder-lake-s.html}},
  year={2022}
}

@inproceedings{fabrication,
  title={7nm vs 10nm vs 14nm: Fabrication Process},
  author={Kashish Kumawat},
  booktitle={\url{https://www.techcenturion.com/7nm-10nm-14nm-fabrication}},
  year={2019}
}

@article{rotem2022intel,
  title={Intel alder lake cpu architectures},
  author={Rotem, Efraim and Yoaz, Adi and Rappoport, Lihu and Robinson, Stephen J and Mandelblat, Julius Yuli and Gihon, Arik and Weissmann, Eliezer and Chabukswar, Rajshree and  others},
  journal={IEEE Micro},
  volume={42},
  number={3},
  pages={13--19},
  year={2022},
  publisher={IEEE}
}

@article{ankur2006noc,
  title={NOC Architecture Design Methodology},
  author={Ankur, Agarwal and Pandya, AS and Abu, Asaduzzaman and Young-Uhg, Lho},
  journal={Journal of the Korea Institute of Information and Communication Engineering},
  volume={10},
  number={1},
  pages={57--64},
  year={2006},
  publisher={The Korea Institute of Information and Commucation Engineering}
}

@article{schoeberl2015t,
  title={T-CREST: Time-predictable multi-core architecture for embedded systems},
  author={Schoeberl, Martin and Abbaspour, Sahar and Akesson, Benny and Audsley, Neil and Capasso, Raffaele and Garside, Jamie and Goossens, Kees and Goossens, Sven and Hansen, Scott and Heckmann, Reinhold and others},
  journal={Journal of Systems Architecture},
  volume={61},
  number={9},
  pages={449--471},
  year={2015},
  publisher={Elsevier}
}

@book{hennessy2011computer,
  title={Computer architecture: a quantitative approach},
  author={Hennessy, John L and Patterson, David A},
  year={2011},
  publisher={Elsevier}
}


@inproceedings{lehoczky1990fixed,
  title={Fixed priority scheduling of periodic task sets with arbitrary deadlines},
  author={Lehoczky, John P},
  booktitle={[1990] Proceedings 11th Real-Time Systems Symposium},
  pages={201--209},
  year={1990},
  organization={IEEE}
}

